OMCAT: Omni Context Aware Transformer

Large Language Models (LLMs) have made significant strides in text generation and comprehension, with recent advancements extending into multimodal LLMs that integrate visual and audio inputs. However, these models continue to struggle with fine-grained, cross-modal temporal understanding, particularly when correlating events across audio and video streams. We address these challenges with two key contributions: a new dataset and model, called OCTAV and OMCAT respectively. OCTAV (Omni Context and Temporal Audio Video) is a novel dataset designed to capture event transitions across audio and video. Second, OMCAT (Omni Context Aware Transformer) is a powerful model that leverages RoTE (Rotary Time Embeddings), an innovative extension of RoPE, to enhance temporal grounding and computational efficiency in time-anchored tasks. Through a robust three-stage training pipeline-feature alignment, instruction tuning, and OCTAV-specific training-OMCAT excels in cross-modal temporal understanding. Our model demonstrates state-of-the-art performance on Audio-Visual Question Answering (AVQA) tasks and the OCTAV benchmark, showcasing significant gains in temporal reasoning and cross-modal alignment, as validated through comprehensive experiments and ablation studies. Our dataset and code will be made publicly available. The link to our demo page is https://om-cat.github.io.

==> introduction.tex <==

% % what's the problem, how we solve it
% Recent times have seen a surge in LLM-based audio and video understanding models that have been used to label data, and to expand LLMs to audio and video.
% These models, however, are limited in their cross-modal understanding, and in their ability to provide answers to questions that are strongly timed or anchored on events. In this paper we address these issues by proposing a new dataset (OVCAT) and a model (OM-CAT). The Omni Context and Temporal Audio Video (OVCAT) dataset does x, y and z. The Omni Context Audio Transformer model (OM-CAT) overcomes the limitations of existing models by doing doing x, y and z. 

% % need for cross-modal models
% Even though there are expert models in audio and video, cross-modality understanding is desirable and necessary because x, y and z. Cross-modal understanding is hard for several reasons, including the lack of cross-modal datasets, unified benchmarks, and understanding on how to combine modalities. Models x, y and z approach it this way but have limitations a, b, c. OM-CAT, on the other hand, addresses these issues though 1, 2, 3.

% % need for strongly-timed and anchored models
% In parallel to these challenges, a strong understanding of the world requires having the ability to provide answers to questions that are strongly timed or anchored on events, Models a, b, c fail at these because 1, 2, 3. We achieve strong-temporal and anchored understanding in OM-CAT by designing a temporal embedding strategy that leverages x, y, z. In addition, because achieving this capabilities requires a dataset that promotes this type of understanding, we propose a method for dataset creation.

% % need for datasets
% Existing audio and video understanding datasets lack the properties x, y, and z. These properties are desirable for audio and video generation models and are required to train audio and video understanding models that  are able to produce answers to strongly timed and anchored questions. As such, we propose a method for dataset creation, that leverages a, b, and c to create datasets. Using this method, we propose the Omni Context and Temporal Audio Video (OCTAV) dataset.

% why multimodal LLMs and progress in current multimodal LLMs
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/figure_1.pdf}
    \vspace{-0.5em}
    \caption{\arushi{modify this figure to include what are the tasks people cureently look at and what is missing}}
    \label{fig.}
\end{figure*}

\arushi{Elaborate here how time is incorporated in video modality separately and audio modality separately, could also discuss more in related work}
Large language models (LLMs) \cite{} have achieved remarkable breakthroughs in both text generation \cite{} and comprehension \cite{} tasks. Since then, significant progress has been made to extend LLMs to multimodal LLMs \cite{}, which integrate visual inputs with textual instructions. These models have set new benchmarks in various fields, including image classification \cite{}, segmentation \cite{}, visual question answering \cite{}, visual grounding \cite{} and so on. More recently, this capability of multimodal LLMs has evolved to comprehend various modalities of audio, videos and text \cite{} to provide understanding in multimodal contexts \cite{}. 
     
% Limitations of current multimodal LLMs
Despite the notable progress in multimodal LLMs \cite{}, most advancements have been centered around high-level tasks like question answering \cite{} and captioning \cite{}, typically within either the video (\eg~Video LLMs \cite{}) or audio (\eg~Audio LLMs \cite{}) domain in isolation. Some efforts have been made towards jointly understanding audio-visual events such as Video LLaMA \cite{}, GroundingGPT \cite{}, MacawLLM \cite{}, AVLLM \cite{} and CAT \cite{}. These models combine audio and video modalities individually as prompts to the LLM. This kind of flexible design can handle multiple modalities simultaneously and achieve competing results on video question answering \cite{}, audio question answering \cite{} and other audio-visual tasks \cite{}. However, these models still face challenges in handling fine-grained, cross-modal temporal understanding when both audio and video are combined. For instance, if a user asks the question, ``Is it raining in the video?'' This question can be answered by either just looking at the video or listening to the audio. However, as shown in \cref{fig.}, if the user asks the question, ``Describe what happens in the video before the sound of dog barking?'', the model needs to understand the cross-correlation between the audio and video modalities as the \texttt{dog barking} cannot be seen in the video and can only be heard and \texttt{what the instructor is doing} cannot be heard in the audio and can only be seen. 

% Specific limitations 
Limited research has been done to address this cross-modal temporal understanding in audio and video modalities. GroundingGPT~\cite{} proposes to predict timestamps but only for the sound events happening in the audio. 
%Simultaneously, they also ground visual regions in the image given the text query. 
It is limited in it's ability to perform cross-modal temporal understanding between the audio and video modalities. AVicuna~\cite{} addresses temporal understanding in both the audio and visual modalities. However, they do not focus on cross-modal temporal understanding as shown in \cref{fig.}. For instance, AVicuna looks at examples such as ``What is the person doing after he is seen dancing from 43 to 83 seconds?'' which requires temporal understanding in videos. However, answering the question ``What is the person doing after the sound of cello?'' requires fine-grained, cross-modal temporal understanding between the audio and video modalities. In this paper, we address this limitation in current multimodal LLMs while achieving competitive/state-of-the-art (?)/significant performance gains on video, audio and audio-video related tasks.   

% What do we exactly do ? 
Our goal is to achieve this cross-modal temporal alignment and to this end we propose \texttt{OM-CAT}, an \textbf{OM}ni \textbf{C}ontext \textbf{A}ware \textbf{T}ransformer. \texttt{OM-CAT} is a unified audio and visual large language model that effectively incorporates time representations to ground the modalities temporally. More specifically, we use rotary position embeddings (RoPE) \cite{}, where we create a unique RoPE embedding for the temporal sequence and apply them to the audio and visual features extracted for that temporal sequence. After applying the RoPE embedding, both the audio and visual features are temporally-aware and aligned by leveraging the continuous nature of RoPE embeddings to handle time dependencies in a smooth manner. For training \texttt{OM-CAT}, we have a feature alignment stage that uses video-text, audio-text and video-audio-text pairs followed by an instruction tuning stage to make \texttt{OM-CAT} aware about time and answer questions in the audio-video domain and learn cross-modal temporal alignment using our proposed instruction tuning dataset.

% Should write about datasets as well that have been designed for these tasks
\arushi{need to write about other instruction tuning datasets}
We propose an instruction tuning dataset, \texttt{OCTAV}: \textbf{O}mni \textbf{C}ontext and \textbf{T}emporal \textbf{A}udio \textbf{V}ideo (\arushi{think about a name}) dataset.\Cref{fig.} shows an example from our proposed \texttt{OCTAV} dataset. Specifically, we create question-answer pairs for a given video such that each question captures the transition between the events happening in the video through a sound event.  For instance, as shown in \cref{fig.}, we add the sound event of \textit{dog barking} to the silent input video between 4 to 10 seconds, during which nothing substantial happens in the video. But we capture the video event before 4 seconds and after 10 seconds while using the dog bark sound as a transition event. This setting encourages the model to not only understand the cross-modal correlation between the audio and video modalities but also a strong temporal understanding of both the audio and video domains in a single setup. \arushi{you can do better in the sentences above.} 
\arushi{add about experimental settings, results and takeaways }
% Our main contributions and takeaways. 
 
In summary, our main contributions are as follows:
\begin{enumerate}
\item Strongly Timed Architecture Design
\item Synthetic Dataset for timed captions
\item "Efficient approach to incorporate time embeddings
    – Improvement on scores
    – Latency is not slow
    – Affect context but rope doesn't"
    \item SOTA on some AV tasks, including timed benchmarks    
\end{enumerate}


==> related_work.tex <==
\vspace{-1em}
\noindent
\textbf{Multimodal LLMs. }Since the development of large language models (LLMs)~\citep{achiam2023gpt,chiang2023vicuna,touvron2023llama}, there has been a growing interest in integrating additional modalities into LLMs~\citep{cheng2024videollama,gong2023listen,kong2024audio}. Video LLMs~\citep{li2023videochat,fu2024video,wang2023internvid} leverage video-text datasets to tackle tasks such as video question answering~\citep{xu2016msr,yu2019activitynet,chen2011collecting}, visual grounding~\citep{kazemzadeh2014referitgame}, and understanding temporal segments in video events~\citep{gao2017tall,huang2024lita}. These models have been further extended to multimodal LLMs~\citep{cheng2024videollama,maaz2023video,lyu2023macaw,su2023pandagpt}, which are capable of encoding multiple modalities, including images, videos, and audio. These models focus on coarse-grained audio-video understanding~\citep{shu2023audio,chen2023valor} and question answering tasks~\citep{yang2022avqa,li2022learning}, achieving notable performance. Despite the advancements in these coarse-grained tasks, these models fall short when it comes to handling fine-grained information in joint audio-visual tasks, where precise synchronization and interpretation of audio and visual modalities are essential for a deeper understanding of events.

There are recent works that try to address this limitation. GroundingGPT~\citep{li2024groundinggpt} predicts fine-grained timestamps, but its focus is limited to sound events within videos, leaving a gap in its understanding of the visual events. On the other hand, AVicuna~\citep{tang2024avicuna} introduces a more balanced approach to temporal understanding in both both audio and visual events. However, both GroundingGPT and AVicuna are limited when it comes to addressing fine-grained, cross-modal temporal understanding, where the interaction between audio and visual modalities is key to understanding complex events over time. Neither of these methods is designed to capture the intricate, interwoven temporal dynamics between audio and video at a highly detailed level, as highlighted in \cref{fig.intro_figure}. This limitation suggests that while progress has been made in multimodal temporal understanding, there is still significant room for improvement in developing models that can fully integrate and align fine-grained cross-modal information, which is the main focus of our work. 
% This would enable more accurate predictions and understanding in complex, real-world scenarios where multiple modalities interact intricately over time.

\noindent
\textbf{Instruction tuning datasets.} The use of large language models (LLMs), particularly GPT models~\citep{achiam2023gpt}, for dataset creation in the domains of video, audio, and audio-video understanding has gained substantial attention. These datasets play a critical role in advancing the capabilities of multimodal models by providing rich, diverse, and large-scale resources to train and evaluate models. In the field of video understanding, GPT-based methods have been employed to generate and annotate large-scale video-text datasets~\citep{wang2023internvid,yang2022learning,luo2023valley,li2023videochat} for video captioning~\citep{fu2024video}, video question answering~\citep{xu2016msr,yu2019activitynet,chen2011collecting}, action recognition~\citep{yu2019activitynet} and so on. For audio understanding, instruction tuning datasets~\citep{kong2024audio, goel2024audio, gong2023listen, chu2023qwen} have been generated to focus on sound events~\citep{salamon2014dataset,fonseca2021fsd50k}, detailed audio captioning~\citep{kim2019audiocaps,mei2024wavcaps,drossos2020clotho}, audio question answering~\citep{lipping2022clotho} \textit{etc.}~More recently, AI-generated datasets have shown great progress in audio-visual models. Instruction based audio-visual datasets~\citep{} are generated~\citep{achiam2023gpt} covering a wide range of mutlimodal tasks such as audio-visual captioning~\citep{chen2023valor,geng2023dense,chen2020vggsound}, question answering~\citep{yang2022avqa,li2022learning} and dialog~\citep{alamri2019audio}. 

Despite the progress made by AI-created datasets, several challenges remain. Current datasets are predominantly coarse-grained, focusing on high-level understanding of audio-visual events. They fail to address tasks that require fine-grained temporal and cross-modal synchronization, such as pinpointing the exact moment an audio event corresponds to a visual cue in complex scenarios. Our proposed dataset, \texttt{OCTAV}, aim to address this limitation in current audio-visual datasets. 
